Feedback Schr\"odinger Bridge Matching

Recent advancements in diffusion bridges for distribution transport problems have heavily relied on matching frameworks, yet existing methods often face a trade-off between scalability and access to optimal pairings during training. Fully unsupervised methods make minimal assumptions but incur high computational costs, limiting their practicality. On the other hand, imposing full supervision of the matching process with optimal pairings improves scalability, however, it can be infeasible in many applications. To strike a balance between scalability and minimal supervision, we introduce Feedback Schr\"odinger Bridge Matching (FSBM), a novel semi-supervised matching framework that incorporates a small portion (less than 8% of the entire dataset) of pre-aligned pairs as state feedback to guide the transport map of non coupled samples, thereby significantly improving efficiency. This is achieved by formulating a static Entropic Optimal Transport (EOT) problem with an additional term capturing the semi-supervised guidance. The generalized EOT objective is then recast into a dynamic formulation to leverage the scalability of matching frameworks. Extensive experiments demonstrate that FSBM accelerates training and enhances generalization by leveraging coupled pairs guidance, opening new avenues for training matching frameworks with partially aligned datasets.

==> Text/Related_Works.tex <==
\section{Extended Review}

\paragraph{Relation Preserving Optimal Transport}
There has been recent advancements in unpaired () or semi-paired (Mustafa and Mantiuk, 2020) data translation, and adaptation of partially paired datasets to guide a conditional score-based diffusion model (Gu et al. (2023)), in order to require fewer source-target aligned image pairs for training, and alleviate the cost of labeling supervised dataset. 
Traditionally, the Gromov-Wasserstein (GW) model (Sturm, 2006; Mémoli, 2011) has been the main approach, aiming to find a “distance-preserving” transport plan where distances between points in the target domain match those in the source domain. A theoretical extension to GW is the TLB (Mémoli, 2011; Sato et al., 2020), a tractable lower bound that uses the ordered distances of each point to all others in the same domain as features. An alternative approach focuses on a “relation-preserving” scheme, maintaining the data's relation to key-points rather than the pairwise distance constraint in GW (Gu et al., 2023).
Furthermore, the concept of the anchors was used to encourage clustering of data and to impose rank constraints on the transport plan to improve its robustness to outliers (Lin et al. (2021)).
These last two lines of work are more closely related to our Semi-Supervised approach, where we try to maintain the relative position that each unlabeled sample had to their respective key-point in the source distribution, throughout the interpolation.
Similar to the notion of clustering presented in Section \ref{}, is Hierarchical distribution steering and OT (Yurochkin et al., 2019; Lee et al., 2019; Xu et al., 2020, Saravanos et al. 2023), where the transportation of points takes place by dividing them into some subgroups. However, it should be underlined that there is no hierarchies in our guidance scheme.\\

\paragraph{Bridge Matching} \cite{peluchetti} first proposed the Markovian projection to propose Bridge Matching (BM), while \cite{liu2022let} applied BM to learn representations in constrained domains.
DSBM (Shi (2023)) employs Iterative Markovian Fitting (IMF) to obtain the Schrodinger Bridge solution. [SF]²M (Tong 2023) provides a simulation-free objective for inferring stochastic dynamics, demonstrating efficiency in solving Schrödinger bridge problems. 

GSBM
(Liu et al., 2023) presents a framework for solving distribution matching to account for task-specific state costs. 
 while Bortoli (2023) explores flow and bridge matching processes, proposing a modification to preserve coupling information, demonstrating efficiency in learning mixtures of image translation tasks.
While these methods aim to identify the optimal coupling, Somnath et al. (2023) and Liu et al. (2023a) propose Bridge Matching algorithms between a priori coupled data, namely the pairing between clean and corrupted images or pairs of biological data from the static Schrödinger Bridge.
Recall that our method recovers DSBM when the guidance is trivial.
The Bridge matching objective offers a computationally efficient alternative but requires additional assumptions. To this front, Action Matching \cite{neklyudov2023action} presents a general matching method with the least assumptions, at the expense of unfavorable to scalability.
Lastly, works that aim to improve the efficiency of these matching frameworks by introducing a light solver for implementing optimal matching using Gaussian mixture parameterization, or proposing a discrete-time counterpart of Iterative Markovian Fitting procedure using Denoising Diffusion GAN for faster generative modeling compared to continuous-time Schrödinger Bridge models (Guschin 2024a, Guschin 2024b). 

\paragraph{Flow Mathching}
On the other hand, when $\sigma\rightarrow 0$, Bridge Matching coincides with Flow Matching (FM) \citep{lipman2022flow} and Conditional Flow Matching (CFM). These methods share the same objective and were developed to train Continuous Normalizing Flows (CNFs) efficiently.
Notably, CFM could be viewed as a generalization of FM, as it offers a stable regression objective for training CNFs without requiring Gaussian source distributions or density evaluations. 
An iterative approach of BM which was proposed by ( Liu et al., 2022) through the concept of the rectified flow, which offers a simple yet effective method for learning ODE models to transport between distributions ( Liu et al., 2022).
This approach resembles Bridge Matching, however, in addition to the deterministic dynamics, another major difference concerns the Markovian projection that takes place only in the forward direction in the context of the Rectified Flow. Consequently, this causes bias to accumulate as the number of iterations increases.
Further developments include Metric Flow Matching (MFM), which learns approximate geodesics on data manifolds ( Kapusniak et al., 2024 ), and Flow Matching in Latent Space, which improves computational efficiency for high-resolution image synthesis ( Dao et al., 2023), training of CNFs on general manifolds (Chen and Lipman 2024). 
Finally, Denoising Diffusion Bridge Models (DDBMs) and the stochastic interpolant unify the framework of flow-based and diffusion-based methods and studied the influence of stochasticity in the bridge, through the concept of stochastic interpolants. (Zhou et al. 2023, Albergo et al. 2023).
